Optimality of Motion Camouflage Under Escape Uncertainty

This letter proposes a novel continuous-time dynamic programming framework to determine when it is optimal for a pursuer to use MC amidst uncertainty in the evader's escape attempt time. We motivate this framework through the model problem of an energy-optimizing male hover fly pursuing a female hover fly for mating. The time at which the female fly initiates an escape is modeled to occur as the result of a non-homogeneous Poisson point process with a biologically informed rate function, and we obtain and solve two Hamilton-Jacobi-Bellman (HJB) PDEs which encode the pursuer's optimal trajectories. Our numerical experiments and statistics illustrate when it is optimal to use MC pursuit tactics amidst uncertainty and how MC optimality is affected by certain properties of the evader's sensing abilities.

==> figs/4pt.tikz.tex <==
% !TEX root = motion_camo_ieee_format.tex

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da07801692851265374] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (72.04,185.67) -- (72.04,51.97) ;
%Straight Lines [id:da8208274790987946] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (170.41,184.34) -- (170.41,50.64) ;
%Straight Lines [id:da9364611126418345] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (120.47,185) -- (120.47,51.31) ;
%Straight Lines [id:da00681963383366635] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (56.15,69.84) -- (184.03,69.84) ;
%Straight Lines [id:da08009135468034012] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (56.53,118.16) -- (184.41,118.16) ;
%Straight Lines [id:da35837057908080916] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (57.67,166.47) -- (185.54,166.47) ;

%Shape: Ellipse [id:dp719802285326707] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (117.73,118.16) .. controls (117.73,116.84) and (118.8,115.78) .. (120.13,115.78) .. controls (121.46,115.78) and (122.54,116.84) .. (122.54,118.16) .. controls (122.54,119.47) and (121.46,120.53) .. (120.13,120.53) .. controls (118.8,120.53) and (117.73,119.47) .. (117.73,118.16) -- cycle ;
%Shape: Ellipse [id:dp1479695146417268] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (118.02,69.51) .. controls (118.02,68.19) and (119.1,67.13) .. (120.43,67.13) .. controls (121.76,67.13) and (122.83,68.19) .. (122.83,69.51) .. controls (122.83,70.82) and (121.76,71.88) .. (120.43,71.88) .. controls (119.1,71.88) and (118.02,70.82) .. (118.02,69.51) -- cycle ;
%Shape: Ellipse [id:dp6544996770838214] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (168,117.49) .. controls (168,116.18) and (169.08,115.12) .. (170.41,115.12) .. controls (171.74,115.12) and (172.81,116.18) .. (172.81,117.49) .. controls (172.81,118.81) and (171.74,119.87) .. (170.41,119.87) .. controls (169.08,119.87) and (168,118.81) .. (168,117.49) -- cycle ;
%Shape: Ellipse [id:dp06151313233394928] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (117.85,166.14) .. controls (117.85,164.83) and (118.93,163.76) .. (120.26,163.76) .. controls (121.59,163.76) and (122.66,164.83) .. (122.66,166.14) .. controls (122.66,167.45) and (121.59,168.52) .. (120.26,168.52) .. controls (118.93,168.52) and (117.85,167.45) .. (117.85,166.14) -- cycle ;
%Shape: Ellipse [id:dp8697825030401247] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (69.3,118.82) .. controls (69.3,117.51) and (70.38,116.44) .. (71.71,116.44) .. controls (73.04,116.44) and (74.11,117.51) .. (74.11,118.82) .. controls (74.11,120.13) and (73.04,121.19) .. (71.71,121.19) .. controls (70.38,121.19) and (69.3,120.13) .. (69.3,118.82) -- cycle ;
%Straight Lines [id:da7270571492649764] 
\draw    (120.43,69.51) -- (170.41,117.49) ;
%Straight Lines [id:da9909713981797195] 
\draw    (71.71,118.82) -- (119.75,69.84) ;
%Straight Lines [id:da5497711650928743] 
\draw    (72.04,118.82) -- (120.26,166.14) ;
%Straight Lines [id:da8781669818603541] 
\draw    (120.26,166.14) -- (170.41,117.49) ;

% Text Node
\draw (91.06,98.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$z_{i,j}$};
% Text Node
\draw (126.11,52.02) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$z_{i,j+1}$};
% Text Node
\draw (172.41,118.52) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$z_{i+1,j}$};
% Text Node
\draw (24.91,116.98) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$z_{i-1,j}$};
% Text Node
\draw (122.26,169.54) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$z_{i,j-1}$};
% Text Node
\draw (124.15,83.05) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {{\fontfamily{pcr}\selectfont 1}};
% Text Node
\draw (107.53,83.05) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {{\fontfamily{pcr}\selectfont 2}};
% Text Node
\draw (107.08,129.61) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {{\fontfamily{pcr}\selectfont 3}};
% Text Node
\draw (122.35,129.61) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {{\fontfamily{pcr}\selectfont 4}};


\end{tikzpicture}

